WorkflowLLM: Enhancing Workflow Orchestration Capability of Large Language Models

Recent advancements in large language models (LLMs) have driven a revolutionary paradigm shift in process automation from Robotic Process Automation to Agentic Process Automation by automating the workflow orchestration procedure based on LLMs. However, existing LLMs (even the advanced OpenAI GPT-4o) are confined to achieving satisfactory capability in workflow orchestration. To address this limitation, we present WorkflowLLM, a data-centric framework elaborately designed to enhance the capability of LLMs in workflow orchestration. It first constructs a large-scale fine-tuning dataset WorkflowBench with 106,763 samples, covering 1,503 APIs from 83 applications across 28 categories. Specifically, the construction process can be divided into three phases: (1) Data Collection: we collect real-world workflow data from Apple Shortcuts and RoutineHub, transcribing them into Python-style code. We further equip them with generated hierarchical thought via ChatGPT. (2) Query Expansion: we prompt ChatGPT to generate more task queries to enrich the diversity and complexity of workflows. (3) Workflow Generation: we leverage an annotator model trained on collected data to generate workflows for synthesized queries. Finally, we merge the synthetic samples that pass quality confirmation with the collected samples to obtain the WorkflowBench. Based on WorkflowBench, we fine-tune Llama-3.1-8B to obtain WorkflowLlama. Our experiments show that WorkflowLlama demonstrates a strong capacity to orchestrate complex workflows, while also achieving notable generalization performance on previously unseen APIs. Additionally, WorkflowBench exhibits robust zero-shot generalization capabilities on an out-of-distribution task planning dataset, T-Eval. Our data and code are available at https://github.com/OpenBMB/WorkflowLLM.

==> section/intro.tex <==

\section{Introduction}
% 第一段： 大模型在若干方面展现出了非常惊人的能力，在很多应用中展现出了应用的价值和潜力，列几个大家熟知的领域，chatdev、具身体
% 第二段： process automation是在干嘛的，定义，目标等。然后补充两到三句详细解释一下，用workflow帮助我们的成果率，让developer面向一个任务设置一个流程，通过人手动开发得到流程，每当有任务的时候，去执行这个workflow。但是workflow的构建是一个人工的过程,耗费专家经验、耗费人力，所以现在有一些工作借助LLM帮助实现LLM，以提升workflow的构建自动化水平。但是现在的工作在plan workflow的方面仍然是不让人满意的。所以现在急需提升大模型在编排workflow上的能力。我们
% 第三段：To address this probelm, 我们提出了WorkflowBench，一个大规模workflow编排SFT数据集。包含多少条数据，多少领域，多少API等等。具体而言，我们的构造过程如下： 1.2.3.。workflow领域统计图，饼状图。两个柱状图，API和workflow的多样性。最终我们在这个数据上finetune得到了一个模型，，参考toolllm.
% 第四段：

% 要提到sft
% llm have achieved remarkable performance
% llm first pretrain on massive data and sft to exlicit their diverse capability
% currently, llm have shown their potential on empowering downstream applications 

Large Language Models~(LLMs), as a new milestone of artificial intelligence, have achieved remarkable performance beyond natural language understanding and generation~\citep{openaichatgptblog,openai2023gpt4,touvron2023llama,dubey2024llama}. 
%
LLMs undergo extensive pretraining on vast datasets to learn fundamental world knowledge and subsequently, the supervised fine-tuning~(SFT) is followed to elicit their versatile capabilities on various tasks~\citep{wei2021finetuned,ouyang2022training}. 
%
Therefore, the advance of LLMs attracts increasing research attentions to empower downstream applications including autonomous agents~\citep{richards2023auto,park2023generative}, software development~\citep{DBLP:conf/acl/QianLLCDL0CSCXL24}, office automation~\citep{DBLP:journals/corr/abs-2407-19056}, data analysis~\citep{ge2024openagi}, and travel planning~\citep{xie2024travelplanner}, embodied AI~\citep{ahn2022can}.

% Large Language Models~(LLMs) have driven significant transformations due to their ability to seamlessly integrate extensive linguistic knowledge with their strong capabilities for invoking external tools and generating code. This advancement has led to remarkable performance across various downstream applications. Moreover, autonomous agents \citep{shen2024hugginggpt,richards2023autogpt} have achieved widespread adoption in domains such as software development \citep{DBLP:conf/acl/QianLLCDL0CSCXL24}, office automation \citep{DBLP:journals/corr/abs-2407-19056}, data analysis \citep{ge2024openagi}, and travel planning \citep{xie2024travelplanner}.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figure/intro.pdf}
    \caption{Overview of our \BenchTitle construction and the derived \ModelName which can develop a workflow based on the user's query (appointment management in this case).}
    \label{fig:intro}
\end{figure}



Process Automation, as a long-standing pursuit of the human race, aims to automate repetitive tasks to minimize human labor and improve productivity and efficiency. 
%
Tracing back to the agricultural era, humanity has employed waterwheels and oxen to automate farming practices.
%
Robotic Process Automation~(RPA), the current predominant process automation technique, abstracts the repetitive task into a workflow (i.e., a program that can execute automatically) by orchestrating various actions (e.g., functions or APIs)~\citep{ivanvcic2019robotic,hofmann2020robotic,wewerka2020robotic,agostinelli2020towards,ferreira2020evaluation}.
%
% abstract repetitive tasks into a unified workflow, thereby minimizing human intervention and significantly improving efficiency. Robotic Process Automation (RPA), a widely adopted automation technology, constructs workflows by orchestrating various actions based on predefined manual rules. 
%
While RPA successfully reduces the need for human labor via automated workflow execution, the process of designing and orchestrating workflows still requires substantial domain expertise and manual effort. 
%
Recently, the emergence of LLMs has unveiled a paradigm shift trend, moving from manual-crafted RPA to LLM-driven Agentic Process Automation~(APA)~\citep{ye2023proagent,zeng2023flowmind,huang2024promptrpa,wornow2024automating,li2024autoflow} which automates the workflow orchestration process by utilizing LLMs to build the workflow. 
%
However, such a potential trend is constrained by the limited ability of LLMs to orchestrate complex workflows, especially for those involving a large number of actions or intricate logical structures including conditions and loops. 
%
% As a representative RPA application, Apple Shortcuts platform has massive workflows which contain $78.1$ actions with a nested logic structure of $3.7$ layers of IF/LOOP on average.
%
Workflows on Apple Shortcuts, a representative widely-used workflow application in the world, average $76.01$ actions.
%
In contrast, ProAgent~\citep{ye2023proagent}, as the proponent of APA, can only orchestrate workflows with $6.1$ actions on average even when equipped with the most advanced OpenAI GPT-4~\citep{openai2023gpt4}, far from meeting the requirements for APA.
%
% As a result, \textbf{there is an urgent need to unlock the workflow orchestration capability of LLMs to expedite the paradigm shift in process automation.}
%
The primary obstacle lies in \textbf{the lack of large-scale SFT datasets for the workflow orchestration task}, resulting in LLMs having unsatisfactory capabilities in this area.
%
As a result, \textbf{there is an urgent need to construct an SFT dataset for workflow orchestration to unlock the capability of LLMs to expedite the paradigm shift in process automation.}

% TODO: 替换数字
To address these challenges, we propose \textbf{\BenchTitle}, a large-scale SFT dataset designed to enhance the capabilities of LLMs in workflow orchestration. 
%
\BenchTitle comprises \TotalNum instruction fine-tuning samples (i.e., workflows), covering \APINum APIs across \APPNum applications. 
%
% Table~\ref{} presents the statistical distribution of these categories. 
%
The construction of \BenchTitle involves three key phases as shown in \Cref{fig:intro}:
%
\begin{itemize}[topsep=-1pt, partopsep=1pt, leftmargin=12pt, itemsep=-1pt]
    \item \textbf{Data Collection}: 
    Apple Shortcuts is a representative application for RPA with massive workflows developed by experts and RoutineHub\footnote{https://routinehub.co} has collected massive real-world Apple shortcuts information, we select them as the high-quality data source.
    %
    We crawled \SeedNum human-annotated high-quality workflows from Apple Shortcuts spanning  \CategoryNum diverse categories (e.g., Business, Health \& Fitness, Productivity, etc) and corresponding metadata from RoutineHub (including shortcut titles, functionality descriptions, API documentations, workflow source codes, etc). 
    %
    % These shortcuts span \CategoryNum diverse categories from RoutineHub, e.g., Business, Health \& Fitness, Productivity, etc.
    %
    % We collected detailed shortcuts information from RoutineHub including shortcut title, functionality description, API documentation, shortcuts source code, etc.
    %
    % Subsequently, we collected APIs from both built-in Apple applications, such as \textit{Safari}, and third-party applications like \textit{OpenAI}, including functionality descriptions, parameter specifications, and return types. 
    %
    % This enhanced the model's ability to learn from documentation and generalize to previously unseen domains. 
    %
    % To resolve the complex syntax of the original data and inconsistencies with the model’s pre-training corpus, we converted both the shortcuts and APIs into Python format.
    %
    % \item \textbf{Data Transformation}:
    %
    As raw workflow data is unsuitable for LLMs to learn, we then transcribe the shortcut source code into Python-style code following~\citet{ye2023proagent}.
    %
    Next, we prompt ChatGPT to generate comments, task plans, and task queries from fine-grained to coarse-grained to provide more detailed thoughts~\citep{wei2023chainofthought} information for LLMs.

    \item \textbf{Query Expansion}:
    To enrich the diversity and complexity of workflows, we utilize ChatGPT to provide more task queries.
    %
    We first sample APPs with diverse functionality and select their APIs together with built-in APIs to prompt ChatGPT to generate task queries that should utilize these sampled APIs to accomplish.
    %
    To ensure the workflow complexity, we further sample real-world workflow samples as demonstrations to prompt ChatGPT to generate similiar ones.

    \item \textbf{Workflow Generation}:
    As existing LLMs even GPT-4o still struggle in workflow generation, we first train a workflow annotator model based on the collected real-world shortcuts data.
    %
    Then we utilize the trained model to generate workflows for the generated task queries.
    %
    % \item \textbf{Quality Confirmation}:
    %
    Due to the low-quality of the generated workflows by the annotator model, we conduct quality confirmation to ensure the dataset quality.
    %
    We first train an evaluator model which can give evaluation scores for the generated workflows and then we filter those with lower scores.
    %
    Next, we utilize ChatGPT to refine the remained workflows to fix existing minor bugs in them.
    %
    Finally, we use rule-based filtering to remove workflows with logical errors.
    

    % \item \textbf{Annotator Model Training}: We prompted \texttt{GPT-4o-mini} to generate instructions, tool-calling plans, and action-level comments using a chain-of-thought approach \citep{wei2022chain} to strengthen the model’s reasoning abilities. We then fine-tuned LLaMA on the seed data to create the annotator model, which we employed to synthesize an expanded dataset more closely aligned with the seed data.

    % \item \textbf{Dataset Expansion}: Given the long-tail distribution of workflow and API categories in the seed data, we expanded the dataset using both ChatGPT and the annotator model. First, we uniformly sampled APIs from the whole set and prompted ChatGPT to generate diverse instructions across various shortcut categories. We then used the annotator model to generate initial tool-calling plans and workflows with comments. Finally, we employed ChatGPT to review these initial responses, correcting grammatical errors and ensuring alignment with the queries, while rule-based methods were used to filter out low-quality samples, such as those with incorrect function call formats.
\end{itemize}

To assess the capability of workflow orchestration, we construct an automatic evaluator model trained on real-world shortcut data.
%
Experimental results show that our constructed evaluator model achieves over $90\%$ evaluation accuracy on the workflow orchestration.
%
We fine-tuned Llama-3.1-8B on our constructed \BenchTitle to derive \ModelName.
%
We conduct experiments on \BenchTitle and find that \ModelName demonstrated strong capabilities in orchestrating complex workflows, outperforming the most advanced LLM, OpenAI GPT-4o.
%
Furthermore, \BenchTitle exhibited robust generalization performance on an out-of-distribution (OOD) setting, T-Eval~\citep{chen2024t}, achieving $77.5\%$ performance.

% To evaluate the workflow orchestration capabilities of LLMs, we employed two assessment methods: (1) CodeBLEU-based evaluation \citep{ren2020codebleu}, which measures not only the syntactic and semantic similarity between the generated workflows and human-annotated ones but also considers the overall functional alignment; and (2) Evaluator-based assessment, where we trained an evaluation model using strong negative samples generated through ChatGPT with in-context learning, along with positive samples from human annotations. Our results demonstrated a close alignment between these evaluation methods and human assessments, offering a robust and scalable approach for evaluating LLM-driven workflow orchestration.


% By fine-tuning LLaMa on \BenchTitle, we obtain \ModelName. After conducting extensive experiments, we found the following: 

% \begin{itemize}[topsep=1pt, partopsep=1pt, leftmargin=12pt, itemsep=-1pt]
% \item \ModelName\ demonstrated strong capabilities in orchestrating complex workflows. As shown in Figure 2, \ModelName\ outperforms both LLaMa3.1 and GPT-4o-mini in the in-context learning setting. Furthermore, \ModelName\ exhibits robust generalization to previously unseen APIs, orchestrating new queries using only the provided API documentation. This adaptability allows the model to scale easily to new APIs, significantly enhancing its practical utility.

% \item We show that both the tool-calling plans and the action-level comments function as intermediate reasoning thoughts that enhance the model's planning capabilities.

% \item \ModelName\ exhibited strong generalization performance on an out-of-distribution (OOD) dataset, T-Eval \citep{chen2024t}. Despite not being trained on T-Eval's APIs or queries, \ModelName\ performed comparably to the powerful closed-source model GPT4o mini.

% \end{itemize}

